SelfDefend: LLMs Can Defend Themselves against Jailbreaking in a Practical Manner

Jailbreaking is an emerging adversarial attack that bypasses the safety alignment deployed in off-the-shelf large language models (LLMs) and has evolved into multiple categories: human-based, optimization-based, generation-based, and the recent indirect and multilingual jailbreaks. However, delivering a practical jailbreak defense is challenging because it needs to not only handle all the above jailbreak attacks but also incur negligible delays to user prompts, as well as be compatible with both open-source and closed-source LLMs. Inspired by how the traditional security concept of shadow stacks defends against memory overflow attacks, this paper introduces a generic LLM jailbreak defense framework called SelfDefend, which establishes a shadow LLM as a defense instance (in detection state) to concurrently protect the target LLM instance (in normal answering state) in the normal stack and collaborate with it for checkpoint-based access control. The effectiveness of SelfDefend builds upon our observation that existing LLMs can identify harmful prompts or intentions in user queries, which we empirically validate using mainstream GPT-3.5/4 models against major jailbreak attacks. To further improve the defense's robustness and minimize costs, we employ a data distillation approach to tune dedicated open-source defense models. When deployed to protect GPT-3.5/4, Claude, Llama-2-7b/13b, and Mistral, these models outperform seven state-of-the-art defenses and match the performance of GPT-4-based SelfDefend, with significantly lower extra delays. Further experiments show that the tuned models are robust to adaptive jailbreaks and prompt injections.

==> This.tex <==
	
	
	
\end{tcolorbox}




\subsection{Extra Delay $\Delta d$}
\label{sec:tundelay}

Similar to how we measured the extra delay $\Delta d$ introduced by GPT-based \name in \mysec\ref{sec:measureresult}, we now report the average delay $\Delta d$ introduced by the tuned models on Llama-2-7b-chat in \myfig~\ref{fig:delay_llama}.
Compared to earlier results in \myfig~\ref{fig:delay}, $\Delta d$ under AlpacaEval is negligible for \name with both $P_{direct}$ and $P_{intent}$, with the former around 0 seconds and the latter around 0.008 seconds.
In contrast, GPT-3.5-based (GPT-4-based) \name with $P_{intent}$ incurred an average $\Delta d$ of around 0.07 seconds (0.02 seconds) under AlpacaEval.
This is likely because the parameters of fine-tuned models are less than those of ChatGPTs.
Besides the normal prompts, the tuned models also significantly reduce the extra delay $\Delta d$ under various jailbreak prompts.
For example, the maximum $\Delta d$ now decreases from the earlier 1.56 seconds on GPT-4 to 0.27 seconds.
Indeed, except for DAN, $\Delta d$ in all attack scenarios are now below 0.1 seconds, while there was no single $\Delta d$ below the same time limit for GPT-4-based \name.
These results indicate that the tuning-based \name achieves negligible delays for both normal and jailbreak prompts, making it feasible for real-world deployment.



\subsection{Explainability}
\label{sec:tunexplain}

\myfig~\ref{fig:gcg}, \ref{fig:pair}, \ref{fig:drattack}, and \ref{fig:multijail} demonstrate the efficacy of the tuned models in identifying harmful content within jailbreak prompts.
Here, we further quantitatively assess whether the identified harmful content actually aligns with the original jailbreak prompt. We measure their semantic similarity using the ensemble CLIP-score~\cite{radford2021learning, zhao2024evaluating, wang2023instructta} as  shown in Table~\ref{tab:exp}.
Note that our measurement exclusively targets the examples where the defense mechanism is successful.


We calculate the CLIP-score between the original prompts $P_{query}$ from JailbreakBench and the attack-generated jailbreak prompts, as well as the CLIP-score between $P_{query}$ and our identified harmful content (prompts/intentions).
%As demonstrated in Table~\ref{tab:exp}, the two CLIP-scores are close, indicating their semantic similarities.
Specifically, the CLIP-scores for identified harmful portions are higher than those for the generated attack prompts, suggesting that the jailbreak prompts have altered the original prompts, whereas the harmful portions identified by our models are more aligned with the original prompts.
Regarding the differences between the two tuned models, we observe that the similarity of identified harmful prompts is higher than that of harmful intentions in the context of human-based, optimization-based, and generation-based attacks, but lower than that of intentions under indirect and multilingual attacks.
This can be attributed to the fact that human-based, optimization-based and generation-based attack prompts contain the original prompts, whereas indirect and multilingual attack prompts significantly distort the original prompts.
In summary, these findings are consistent with our initial design intentions and demonstrate that the harmful portions identified by our models can indeed provide an explainable foundation for defense mechanisms.




\input{robust}





%\begin{table*}[t]
%	\centering
%	\caption{Jailbreak pass rates of various defense methods for GPT-3.5.}
%	\resizebox{\textwidth}{!}{
%		\begin{tabular}{l|cc|cc|cc|c|c}
%			\toprule
%			\multirow{2}{*}{Defense Method} & \multicolumn{2}{c|}{Optimization-based} & \multicolumn{2}{c|}{Template-based} &\multicolumn{2}{c|}{Indirect} &Multilingual & Normal \\ \cline{2-9}
%			& GCG & JSAA & PAIR & AutoDAN & DrAttack & Puzzler & MultiJail & AlpacaEval   \\ \hline
%			GPT-3.5  & 0.56 & 0.94 & 0.72 & 0.90 & 0.78 & 0.98 & 0.39 & 0.97  \\
%			Perplexity Filter \cite{jain2023baseline}  & \textbf{0.03} & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.99 \\
%			SmoothLLM \cite{SmoothLLM2310}    & 0.48 & 0.89 & 0.65 & 0.93 & 0.85 & 0.99 & 1.00 & 0.96   \\
%			{Llama Guard} \cite{LlamaGuard2312}   & 0.41 & 0.61 & 0.43 & 1.00 & 0.97 & 0.93 & 0.95 & 0.99   \\
%			{Llama Guard 2} \cite{metallamaguard2}  & 0.14 & 0.50 & 0.37 & 0.15 & 0.89 & 0.64 & 0.55 & 0.99  \\ \hline
%			shadow stack (direct prompt) & 0.08 & 0.11 & 0.14 & \textbf{0.07} & 0.78 & \textbf{0.07} & 0.74 & 0.96   \\
%			SelfDefend (direct prompt)  & 0.06 & 0.11 & \textbf{0.07} & \textbf{0.07} & 0.62 & \textbf{0.07} & 0.30 & 0.94   \\
%			shadow stack (intent prompt)  & 0.08 & \textbf{0.05} & 0.16 & 0.09 & 0.18 & 0.20 & 0.57 & 0.99   \\
%			SelfDefend (intent prompt) & 0.05 & \textbf{0.05} & 0.12 & 0.08 & \textbf{0.16} & 0.20 & \textbf{0.26} & 0.97  \\
%			\bottomrule
%		\end{tabular}
%	}
%	\label{tab:tuning_gpt35}
%\end{table*}
%
%\begin{table*}[t]
%	\centering
%	\caption{Jailbreak pass rates of various defense methods for GPT-4.}
%	\resizebox{\textwidth}{!}{
%		\begin{tabular}{l|cc|cc|cc|c|c}
%			\toprule
%			\multirow{2}{*}{Defense Method} & \multicolumn{2}{c|}{Optimization-based} & \multicolumn{2}{c|}{Template-based} &\multicolumn{2}{c|}{Indirect} &Multilingual & Normal \\ \cline{2-9}
%			& GCG & JSAA & PAIR & AutoDAN & DrAttack & Puzzler & MultiJail & AlpacaEval   \\ \hline
%			GPT-4   & 0.08 & 0.16 & 0.33 & 0.19 & 0.74 & 0.90 & 0.08 & 0.97  \\
%			{Perplexity Filter} \cite{jain2023baseline}  & 0.03 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.99  \\
%			{SmoothLLM} \cite{SmoothLLM2310}    & 0.07 & 0.19 & 0.33 & 0.18 & 0.91 & 0.88 & 1.00 & 0.97   \\
%			{Llama Guard} \cite{LlamaGuard2312}   & 0.41 & 0.61 & 0.43 & 1.00 & 0.98 & 0.93 & 0.95 & 0.99    \\
%			{Llama Guard 2} \cite{metallamaguard2}  & 0.14 & 0.50 & 0.35 & 0.15 & 0.91 & 0.64 & 0.55 & 0.99   \\ \hline
%			shadow stack (direct prompt)  & 0.04 & 0.11 & 0.17 & 0.07 & 0.71 & 0.12 & 0.71 & 0.96    \\
%			SelfDefend (direct prompt)   & \textbf{0.01} & 0.07 & \textbf{0.15} & \textbf{0.05} & 0.58 & \textbf{0.07} & 0.06 & 0.94   \\
%			shadow stack (intent prompt) & 0.08 & 0.03 & 0.19 & 0.07 & 0.18 & 0.19 & 0.56 & 0.99    \\
%			SelfDefend (intent prompt)  & 0.04 & \textbf{0.02} & 0.19 & 0.06 & \textbf{0.17} & 0.14 & \textbf{0.04} & 0.97   \\
%			\bottomrule
%		\end{tabular}
%	}
%	\label{tab:tuning_gpt4}
%\end{table*}
%
%\begin{table*}[t]
%	\centering
%	\caption{Jailbreak pass rates of multiple defense methods based on LLaMA-2-7b-chat.}
%	\resizebox{1.0\textwidth}{!}{
%		\begin{tabular}{l|cc|cc|cc|c|c}
%			\toprule
%			\multirow{2}{*}{Defense Method} & \multicolumn{2}{c|}{Optimization-based} & \multicolumn{2}{c|}{Template-based} &\multicolumn{2}{c|}{Indirect} &Multilingual & Normal \\ \cline{2-9}
%			& GCG & JSAA & PAIR & AutoDAN & DrAttack & Puzzler & MultiJail & AlpacaEval   \\ \hline
%			LLaMA-2-7b-chat                             & 0.57 & 0.96 & 0.59 & 0.68 & 0.88 & 0.99 & 0.14 & 0.98  \\
%			{Perplexity Filter} \cite{jain2023baseline} & \textbf{0.00} & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.99  \\
%			{SmoothLLM} \cite{SmoothLLM2310}            & 0.93 & 1.00 & 0.82 & 0.95 & 0.98 & 1.00 & 0.99 & 0.99  \\
%			{Llama Guard} \cite{LlamaGuard2312}         & 0.40 & 0.41 & 0.46 & 1.00 & 0.84 & 0.93 & 0.95 & 0.99  \\
%			{Llama Guard 2} \cite{metallamaguard2}      & 0.17 & 0.53 & 0.41 & 0.15 & 0.89 & 0.64 & 0.55 & 0.99  \\ \hline
%			shadow stack (direct prompt)                & 0.06 & 0.06 & 0.25 & \textbf{0.05} & 0.36 & \textbf{0.09} & 0.73 & 0.97  \\
%			SelfDefend (direct prompt)                  & 0.04 & 0.06 & 0.22 & \textbf{0.05} & 0.31 & \textbf{0.09} & 0.10 & 0.95  \\
%			shadow stack (intent prompt)                & 0.11 & \textbf{0.02} & 0.24 & 0.08 & \textbf{0.15} & 0.22 & 0.58 & 0.99  \\
%			SelfDefend (intent prompt)                  & 0.09 & \textbf{0.02} & \textbf{0.21} & 0.07 & \textbf{0.15} & 0.22 & \textbf{0.06} & 0.98  \\
%			\bottomrule
%		\end{tabular}
%	}
%	\label{tab:tuning_llama}
%\end{table*}



%\begin{table*}[t]
%	\centering
%	\caption{Defense performance on GPT-3.5.}
%	\resizebox{0.99\textwidth}{!}{
%		\begin{tabular}{l|cccccc|cccccc}
%			\toprule
%			\multirow{2}{*}{Defense Method} & \multicolumn{6}{c|}{ASR ($\downarrow$)} & \multicolumn{6}{c}{Delay ($\downarrow$)} \\ \cline{2-13}
%			& GCG & JSAA & PAIR & AutoDAN & DrAttack & Puzzler & GCG & JSAA & PAIR & AutoDAN & DrAttack & Puzzler  \\ \hline
%			GPT-3.5  & 0.56 & 0.94 & 0.72 & 0.90 & 0.78 & 0.98 & 1.61 & 2.05 & 1.85 & 2.00 & 2.05 & 2.11  \\
%			Perplexity Filter  & \textbf{0.03} & & 1.00 & 1.00 & 1.00 & 1.00 & 0.06 & & 0.11 & 0.13 & 0.36 & 1.54  \\
%			SmoothLLM     & 0.48 & X & 0.65 & 0.93 & 0.85 & 0.99 & 20.49 & X & 21.08 & 25.72 & 24.88 & 22.28   \\
%			{Llama Guard}   & 0.41 & X & 0.43 & 1.00 & 0.97 & 0.93 & 0.26 & X & 0.27 & 0.21 & 0.28 & 1.04   \\
%			{Llama Guard 2}  & 0.14 & X & 0.37 & 0.15 & 0.89 & 0.64 & 0.18 & X & 0.15 & 0.18 & 0.16 & 0.41  \\ \hline
%			P1                  & 0.11 & X & 0.13 & 0.00 & 0.74 & \textbf{0.10} & 0.87 & X & 1.02 & 0.21 & 0.71 & 3.58   \\
%			GPT-3.5 + P1  & 0.07 & X & \textbf{0.09} & 0.00 & 0.63 & \textbf{0.10} & 1.65 & X & 1.89 & 2.00 & 2.25 & 3.78   \\
%			P2                  & 0.08 & X & 0.18 & 0.00 & 0.27 & 0.19 & 1.95 & X & 2.08 & 0.25 & 2.15 & 4.11   \\
%			GPT-3.5 + P2  & 0.05 & X & 0.14 & 0.00 & \textbf{0.24} & 0.19 & 2.05 & X & 2.22 & 2.00 & 2.45 & 4.13  \\
%			\bottomrule
%		\end{tabular}
%	}
%	\label{tab:tuning_gpt35}
%\end{table*}
%
%
%\begin{table*}[t]
%	\centering
%	\caption{Defense performance on GPT-3.5.}
%	\resizebox{0.99\textwidth}{!}{
%		\begin{tabular}{l|cccccc|cccccc}
%			\toprule
%			\multirow{2}{*}{Defense Method} & \multicolumn{6}{c|}{ASR ($\downarrow$)} & \multicolumn{6}{c}{Delay ($\downarrow$)} \\ \cline{2-13}
%			& GCG & JSAA & PAIR & AutoDAN & DrAttack & Puzzler & GCG & JSAA & PAIR & AutoDAN & DrAttack & Puzzler  \\ \hline
%			GPT-4   & 0.08 & & 0.33 & 0.19 & 0.74 & 0.90 & 1.43 & & 2.44 & 1.70 & 3.90 & 4.79  \\
%			{Perplexity Filter}  & 0.03 & & 1.0 & 1.00 & 1.00 & 1.00 & 0.06 & & 0.11 & 0.13 & 0.38 & 1.53  \\
%			{SmoothLLM}     & & X & & & & & & X & & & &   \\
%			{Llama Guard}   & & X & & & & & & X & & & &   \\
%			{Llama Guard 2}  & & & & & & & & & & & &  \\ \hline
%			P1  & & X & & & & & & X & & & &   \\
%			GPT-3.5 + P1  & & X & & & & & & X & & & &   \\
%			P2  & & X & & & & & & X & & & &   \\
%			GPT-3.5 + P2  & & X & & & & & & X & & & &   \\
%			\bottomrule
%		\end{tabular}
%	}
%	\label{tab:tuning_gpt4}
%\end{table*}


==> futuredirection.tex <==
\section{Future Directions}
\label{sec:direction}


While \name is promising, there are several future research directions to make it fully practical in a real-world setting, as illustrated in \myfig~\ref{fig:overview}.


\begin{itemize}
    \item \textbf{FD1:} \textit{Design a low-cost, fast, and robust LLM for accurately recognizing harmful prompts.}
        While existing GPT-3.5/4 models already perform well in recognizing harmful prompts, it is desirable to reduce their inference cost and improve their inference speed. Moreover, we need a robust LLM that can accurately recognize harmful prompts in various adversarial scenarios. In particular, it needs to prevent potential prompt injection attacks~\cite{PromptInjection2310} launched by adversaries who are aware of \name's defense.
        To robustly defend against prompt injection, one approach is to leverage prefix tuning~\cite{PrefixTuning21} so that our detection prompt, shown in \myfig~\ref{fig:overview}, is integrated into LLMs as a prefix rather than a potentially manipulable prompt.

    \item \textbf{FD2:} \textit{Use the discovered AEs to further align LLMs.}
        By cross-checking the response given by LLMs, \name can also identify jailbreak prompts as AEs (adversarial examples) that can bypass existing alignment.
        These AEs can be used to further align the safety of LLMs.
        A better-aligned LLM in the normal stack can also enhance the detection of harmful prompts in the shadow stack.
        That said, by investigating the additional token-by-token output available when a checkpoint is triggered, we can confirm whether a harmful prompt has been identified in the shadow stack.
        We plan to conduct an ablation study to verify this.

    \item \textbf{FD3:} \textit{Design mechanisms to reduce/cache the calling of shadow stack.}
        In \name's original design, every user prompt needs to go through the checking process in the shadow stack, which could be enhanced by a caching mechanism.
        Therefore, another direction is how to design effective caching mechanisms for the shadow stack in a real-world setting.
\end{itemize}


Besides the research directions listed above, a valuable extension of \name is to support defense against multimodal jailbreak.
While \name can immediately defend against multimodal jailbreaks with harmful text prompts~\cite{VisualJailbreak2306, JailbreakGPT4V2311, JailbreakMultimodal2402}, it, by design, cannot handle pure multimodal jailbreaks~\cite{ImageSoundJailbreak2307} that use only images or sounds without any harmful text prompts~\cite{VRPTEST2312}.
A revised design of \name should be explored to defend against such advanced multimodal jailbreaks~\cite{ImageSoundJailbreak2307}.


==> lessons.tex <==
\subsection{Lessons Learned}
\label{sec:lessons}



==> threat.tex <==
\subsection{Threat to Validity and Limitations}
\label{sec:threat}



